Improving the Efficiency of Human-in-the-Loop Systems: Adding Artificial to Human Experts

Information systems increasingly leverage artificial intelligence (AI) and machine learning (ML) to generate value from vast amounts of data. However, ML models are imperfect and can generate incorrect classifications. Hence, human-in-the-loop (HITL) extensions to ML models add a human review for instances that are difficult to classify. This study argues that continuously relying on human experts to handle difficult model classifications leads to a strong increase in human effort, which strains limited resources. To address this issue, we propose a hybrid system that creates artificial experts that learn to classify data instances from unknown classes previously reviewed by human experts. Our hybrid system assesses which artificial expert is suitable for classifying an instance from an unknown class and automatically assigns it. Over time, this reduces human effort and increases the efficiency of the system. Our experiments demonstrate that our approach outperforms traditional HITL systems for several benchmarks on image classification.

==> Tables/bench_models_implementation_details.tex <==
\begin{sidewaystable}[H]
\centering

\begin{subtable}[H]{1\textwidth}
\centering
\scalebox{0.83}{
\begin{tabular}{l
>{\raggedright\arraybackslash}p{3.15cm}%
|cccc
>{\centering\arraybackslash}p{4cm}%
>{\centering\arraybackslash}p{4cm}%
>{\centering\arraybackslash}p{2cm}%
}

\toprule
\textbf{Domain} & \textbf{Model} & Architecture & Batch size & Epochs & Loss function & Optimizer (learning rate / weight decay / momentum) & Learning rate scheduler & Early stopping \\
\midrule
single + multi & CIFAR-10 & WRN-28-10 & 256 & 200 & CrossEntropyLoss & SGD(0.1/0.0001/0.9) & CosineAnealling & no  \\
multi & SVHN & WRN-28-10 & 256 & 100 & CrossEntropyLoss & SGD(0.1/0.0001/0.9) & ReduceOnPlateau & no \\
multi & MNIST & WRN-28-10 & 256 & 20 & CrossEntropyLoss & SGD(0.1/0.0001/0.9) & CosineAnealling & no \\
multi & Fashion-MNIST & WRN-28-10 & 128 & 300 & CrossEntropyLoss & SGD(0.1/0.0005/0.9) & Individual approach & no \\
multi & Gating & DenseNet-121 & 256 & 3 & CrossEntropyLoss & SGD(0.1/0/-) & ReduceOnPlateau & no \\
multi & Global & WRN-28-10 & 256 & 300 & CrossEntropyLoss & SGD(0.1/0.0001/0.9) & ReduceOnPlateau & no \\

\bottomrule
\end{tabular}}
\caption{Static AI-in-the-Loop-system}
\label{bench_static}
\end{subtable}

\vspace{1cm}

\begin{subtable}[H]{1\textwidth}
\centering

\scalebox{0.83}{
\begin{tabular}{l
>{\raggedright\arraybackslash}p{3.15cm}%
|cccc
>{\centering\arraybackslash}p{4cm}%
>{\centering\arraybackslash}p{4cm}%
>{\centering\arraybackslash}p{2cm}%
}

\toprule
\textbf{Domain} & \textbf{Model} & Architecture & Batch size & Epochs & Loss function & Optimizer (learning rate / weight decay / momentum) & Learning rate scheduler & Early stopping \\
\midrule
single + multi & CIFAR-10 & WRN-28-10 & 256 & 200 & CrossEntropyLoss & SGD(0.1/0.0001/0.9) & CosineAnealling & no \\
multi & SVHN/MNIST/ \newline Fashion-MNIST & WRN-28-10 & 128 & 300 & CrossEntropyLoss & SGD(0.1/0.0001/0.9) & ReduceOnPlateau & yes \\
multi & Gating & DenseNet-121 & 256 & 3 & CrossEntropyLoss & SGD(0.1/0/-) & ReduceOnPlateau & no \\


\bottomrule
\end{tabular}}
\caption{Dynamic AI-in-the-Loop-system}
\label{bench_dynamic}
\end{subtable}

\caption{Training parameters of the ML models in the benchmark case (single-domain seed: 438636; multi-domain seed: 855325)}.
\label{bench_models_implementation}
\end{sidewaystable}

==> Tables/bench_multi_dynamic_maha31_allomatrix.tex <==
\begin{table}[H]
\centering

\scalebox{0.75}{

\begin{tabular}{l
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
}


\toprule
& \multicolumn{6}{c}{Allocation} \\
\cline{2-7}
{} &  \textbf{Gen. model} &   \textbf{Exp. 1} &  \textbf{Exp. 2} &  \textbf{Exp. 3} & \textbf{Human exp.} &   \textbf{Total} \\
\midrule
\textbf{Gen. model             } &   \textbf{159} &       0 &       0 &       0 &     \multicolumn{1}{r|}{2}  &   161 \\
\textbf{Exp. 1           } &   210 &    \textbf{2187} &       0 &       0 &   \multicolumn{1}{r|}{211} &  2608 \\
\textbf{Exp. 2           } &     0 &       7 &     \textbf{822} &      50 &  \multicolumn{1}{r|}{1287} &  2166 \\
\textbf{Exp. 3           } &   114 &      33 &       0 &     \textbf{729} &  \multicolumn{1}{r|}{1290} &  2166 \\
\hline
\textbf{Total                 } &   483 &    2227 &     822 &     779 &  \multicolumn{1}{r|}{2790} &  7101 \\
\hline
\hline
\textbf{Coverage            } &     0.07 &       0.31 &       0.12 &       0.11 &     \multicolumn{1}{r|}{0.39} &     - \\
\textbf{Perfect coverage    } &     0.02 &       0.36 &       0.31 &       0.31 &     \multicolumn{1}{r|}{0.00} &     - \\
\hline
\textbf{Claimed data accuracy} &     0.32 &       0.92 &       0.97 &       0.89 &     \multicolumn{1}{r|}{1.00} &     - \\
\textbf{Testset accuracy     } &        0.96 &     0.95 &    0.96 &    0.93 &        \multicolumn{1}{r|}{1.00} &     - \\
\bottomrule
\end{tabular}}
\caption{Allocation of data samples and accuracies of the general model, the artificial experts and the human expert in batch number 31 of the dynamic, multi-domain AI-in-the-Loop-system deploying the Maha allocation mechanism in the benchmark case.}
\label{benchmark_multi_dynamic_allomatrix}
\end{table}


==> Tables/bench_multi_static_allomatrices.tex <==
\begin{table}
\centering

\begin{subtable}[H]{1\textwidth}
\centering
\scalebox{0.75}{
\begin{tabular}{l
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
}
\toprule
& \multicolumn{6}{c}{Allocation} \\
\cline{2-7}
{} &  \textbf{Gen. model} &   \textbf{Exp. 1} &  \textbf{Exp. 2} &  \textbf{Exp. 3} & \textbf{Human exp.} &   \textbf{Total} \\
\midrule
\textbf{Gen. model          } &      \textbf{159} &     1 &     0 &     0 &         \multicolumn{1}{r|}{1} &   161 \\
\textbf{Exp. 1              } &        0 &  \textbf{2608} &     0 &     0 &         \multicolumn{1}{r|}{0} &  2608 \\
\textbf{Exp. 2              } &        0 &     0 &  \textbf{2166} &     0 &         \multicolumn{1}{r|}{0} &  2166 \\
\textbf{Exp. 3              } &        0 &     0 &     0 &  \textbf{2166} &         \multicolumn{1}{r|}{0} &  2166 \\
\hline
\textbf{Total               } &      159 &  2609 &  2166 &  2166 &         \multicolumn{1}{r|}{1} &  7101 \\
\hline
\hline
\textbf{Coverage            } &        0.02 &     0.36 &     0.31 &     0.31 &         \multicolumn{1}{r|}{0.00} &     - \\
\textbf{Perfect coverage    } &        0.02 &     0.36 &     0.31 &     0.31 &         \multicolumn{1}{r|}{0.00} &     - \\
\hline
\textbf{Claimed data accuracy} &        0.97 &     0.96 &     0.98 &     0.96 &         \multicolumn{1}{r|}{1.00} &     - \\
\textbf{Testset accuracy     } &        0.96 &    0.97 &     0.98 &    0.96 &        \multicolumn{1}{r|}{1.00} &     - \\

\bottomrule
\end{tabular}}
\caption{$\Psi_1, \Psi_2$ = Gating}
\label{bench_gating}
\end{subtable}

\vspace{1cm}

\begin{subtable}[H]{1\textwidth}
\centering

\scalebox{0.75}{
\begin{tabular}{l
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
}
\toprule
& \multicolumn{6}{c}{Allocation} \\
\cline{2-7}
{} &  \textbf{Gen. model} &   \textbf{Exp. 1} &  \textbf{Exp. 2} &  \textbf{Exp. 3} & \textbf{Human exp.} &   \textbf{Total} \\
\midrule
\textbf{Gen. model          } &      \textbf{161} &     0 &     0 &     0 &        \multicolumn{1}{r|}{0} &   161 \\
\textbf{Exp. 1              } &      172 &  \textbf{2309} &     0 &     0 &      \multicolumn{1}{r|}{127} &  2608 \\
\textbf{Exp. 2              } &        0 &    19 &  \textbf{1476} &     0 &      \multicolumn{1}{r|}{671} &  2166 \\
\textbf{Exp. 3              } &       98 &    16 &     0 &  \textbf{1247} &      \multicolumn{1}{r|}{805} &  2166 \\
\hline
\textbf{Total               } &      431 &  2344 &  1476 &  1247 &     \multicolumn{1}{r|}{1603} &  7101 \\
\hline
\hline
\textbf{Coverage            } &        0.06 &     0.33 &     0.21 &     0.18 &        \multicolumn{1}{r|}{0.23} &     - \\
\textbf{Perfect coverage    } &        0.02 &     0.36 &     0.31 &     0.31 &        \multicolumn{1}{r|}{0.00} &     - \\
\hline
\textbf{Claimed data accuracy} &        0.36 &     0.96 &     0.99 &     0.98 &        \multicolumn{1}{r|}{1.00} &     - \\
\textbf{Testset accuracy     } &        0.96 &    0.97 &     0.98 &    0.96 &        \multicolumn{1}{r|}{1.00} &     - \\

\bottomrule
\end{tabular}}
\caption{$\Psi_1, \Psi_2$ = Maha}
\label{bench_maha}
\end{subtable}
\vspace{1cm}

\begin{subtable}[H]{1\textwidth}
\centering

\scalebox{0.75}{
\begin{tabular}{l
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
>{\raggedleft\arraybackslash}p{1.5cm}%
}
\toprule
& \multicolumn{6}{c}{Allocation} \\
\cline{2-7}
{} &  \textbf{Gen. model} &   \textbf{Exp. 1} &  \textbf{Exp. 2} &  \textbf{Exp. 3} & \textbf{Human exp.} &   \textbf{Total} \\
\midrule
\textbf{Gen. model          } &      \textbf{150} &    0 &    6 &    0 &        \multicolumn{1}{r|}{5} &   161 \\
\textbf{Exp. 1              } &      177 &  \textbf{154} &  114 &    0 &     \multicolumn{1}{r|}{2163} &  2608 \\
\textbf{Exp. 2              } &      747 &   13 &  \textbf{786} &    1 &      \multicolumn{1}{r|}{619} &  2166 \\
\textbf{Exp. 3              } &      576 &    0 &   80 &  \textbf{137} &     \multicolumn{1}{r|}{1373} &  2166 \\
\hline
\textbf{Total               } &     1650 &  167 &  986 &  138 &     \multicolumn{1}{r|}{4160} &  7101 \\
\hline
\hline
\textbf{Coverage            } &        0.23 &    0.02 &    0.14 &    0.02 &        \multicolumn{1}{r|}{0.59} &     - \\
\textbf{Perfect coverage    } &        0.02 &    0.36 &    0.31 &    0.31 &        \multicolumn{1}{r|}{0.00} &     - \\
\hline
\textbf{Claimed data accuracy} &        0.09 &    0.90 &    0.79 &    0.95 &        \multicolumn{1}{r|}{1.00} &     - \\
\textbf{Testset accuracy     } &        0.96 &    0.97 &     0.98 &    0.96 &        \multicolumn{1}{r|}{1.00} &     - \\


\bottomrule
\end{tabular}}
\caption{$\Psi_1, \Psi_2$ = ODIN}
\label{bench_odin}
\end{subtable}

\caption{Allocation of data samples and accuracies of the general model, the artificial experts and the human expert of the static, multi-domain AI-in-the-Loop-system deploying different allocation mechanisms in the benchmark case.}
\label{benchmark_multi_static_allomatrix}
\end{table}

==> Tables/bench_multi_static_combos.tex <==
\begin{table}
\centering

\begin{subtable}[h]{1\textwidth}
\centering

\scalebox{0.75}{
\begin{tabular}{lc@{\hskip 20pt}c@{\hskip 20pt}c@{\hskip 20pt}c@{\hskip 20pt}c}
\toprule
\textbf{$\Psi_1$ / $\Psi_2$} & \textbf{Gating} & \textbf{Maha} & \textbf{ODIN$_{int}$} & \textbf{ODIN} & \multicolumn{1}{c}{\textbf{\textcolor{gray}{Softmax}}} \\
\midrule

% HIER KOMMT DIE METRIK ÜBERSICHT
 & \multicolumn{5}{c}{Accuracy / Human coverage / Utility score ($\alpha=1.0$, $\beta=0.5$)} \\
\cline{2-6}


\textbf{Gating           } &  0.97/\textbf{0.00}/\textbf{0.97} &  
\textbf{0.98}/0.23/0.86 & 0.96/0.71/0.60 & 0.96/0.72/0.60 &      \textcolor{gray}{0.79/0.00/0.79} \\

\textbf{Maha             } &  0.93/\textbf{0.00}/0.93 &  
0.94/0.23/0.83 & 0.92/0.68/0.58 & 0.92/0.69/0.58 &
\textcolor{gray}{0.76/0.00/0.76} \\
\textbf{ODIN$_{int}$            } &  0.76/\textbf{0.00}/0.76 & 
0.77/0.17/0.69 & 0.76/0.58/0.46 & 0.76/0.59/0.46 & 
\textcolor{gray}{0.61/0.00/0.61} \\
\textbf{ODIN} &  0.76/\textbf{0.00}/0.76 & 
0.77/0.17/0.69 & 0.76/0.58/0.46 & 0.76/0.59/0.46 & 
\textcolor{gray}{0.61/0.00/0.61} \\
%\cline{1-5}
\textbf{\textcolor{gray}{Softmax}       } &  \textcolor{gray}{0.80/0.00/0.80} & 
\textcolor{gray}{0.81/0.18/0.72} & 
\textcolor{gray}{0.79/0.61/0.49} & \textcolor{gray}{0.79/0.60/0.49} & 
\textcolor{gray}{0.64/0.00/0.64} \\
\bottomrule
\end{tabular}}
\caption{Overview of combinations}
\end{subtable}

\begin{subtable}[h]{1\textwidth}
\centering

\vspace{0.5cm}
\scalebox{0.75}{

\begin{tabular}{l
>{\centering\arraybackslash}p{6cm}%
}
\toprule
& Accuracy /\newline Human coverage /\newline Utility score ($\alpha=1.0$, $\beta=0.5$) \\
\midrule
\textbf{General model       } & 0.02/0.00/0.02 \\
\textbf{Random allocation } & 0.33/0.00/0.33 \\
\textbf{Global model             } & 0.97/0.00/0.97 \\
\textbf{Perfect allocation} & 0.97/0.00/0.97 \\
\textbf{HITL-system     } & 1.00/0.98/0.51 \\
\bottomrule
\end{tabular}}
\caption{Baselines}
\label{benchmark_multi_static_baselines}
\end{subtable}


\caption{Overview of the accuracy, the human coverage and the utility score ($\alpha=1.0$, $\beta=0.5$) of all allocation mechanism combinations and baselines of the static, multi-domain AI-in-the-Loop-system in the benchmark case.}
\label{benchmark_multi_static_combos}
\end{table}



==> Tables/bench_single_dynamic_acc_cov.tex <==
\begin{table}
\centering

\scalebox{0.75}{

\begin{tabular}{lcc|
>{\centering\arraybackslash}p{2cm}%
>{\centering\arraybackslash}p{2cm}%
>{\centering\arraybackslash}p{2cm}%
}

\toprule
\textbf{} & & \textbf{Softmax} & \textbf{General model} & \textbf{HITL-system} & \textbf{Perfect coverage} \\
\textbf{Batch} &     1 &      31 &              31 &                31 &               31 \\
\midrule
\textbf{Gen. model coverage} &  0.40 &    0.37 &            1.00 &              0.20 &             0.25 \\
\textbf{Exp. 1 coverage    } &  0.00 &    0.55 &            0.00 &              0.00 &             0.75 \\
\textbf{Human coverage     } &  0.60 &    0.08 &            0.00 &              0.80 &             0.00 \\
\textbf{Accuracy       } &  0.75 &    0.75 &            0.18 &              0.98 &             0.00 \\
\bottomrule
\end{tabular}

}
\caption{Overview of the coverages and the accuracy of the dynamic, single-domain AI-in-the-Loop-system in the benchmark case.}
\label{benchmark_single_dynamic_acc_cov}
\end{table}


